Real Time Multi Organ Classification on Computed Tomography Images

Organ segmentation is a fundamental task in medical imaging since it is useful for many clinical automation pipelines. However, some tasks do not require full segmentation. Instead, a classifier can identify the selected organ without segmenting the entire volume. In this study, we demonstrate a classifier based method to obtain organ labels in real time by using a large context size with a sparse data sampling strategy. Although our method operates as an independent classifier at query locations, it can generate full segmentations by querying grid locations at any resolution, offering faster performance than segmentation algorithms. We compared our method with existing segmentation techniques, demonstrating its superior runtime potential for practical applications in medical imaging.

==> sec/gptfeedback.tex <==
Performance Metrics: Providing a more detailed comparison in terms of both speed and accuracy across a broader range of existing methods. Highlight how the proposed method performs under different scenarios, potentially including challenging cases where current methods underperform.


Trade-offs and Limitations: Clearly discussing the trade-offs involved in using the proposed sparse sampling method versus more traditional approaches. For instance, while the method might achieve faster processing times, how does it handle complex medical scenarios where high accuracy and precision are critical?

Error Analysis: Incorporating an error analysis would significantly strengthen the paper. This section should detail the conditions under which the proposed method may fail or produce lower accuracy, helping to set realistic expectations for its application.
Use Cases and Practicality: Expanding on how this method could be integrated into current medical imaging workflows. Practical demonstrations or pilot studies showing the method in use, discussing its integration with existing technologies, and feedback from actual clinical environments would greatly enhance the paper's impact.
